4D Gaussian Splatting as a Learned Dynamical System

We reinterpret 4D Gaussian Splatting as a continuous-time dynamical system, where scene motion arises from integrating a learned neural dynamical field rather than applying per-frame deformations. This formulation, which we call EvoGS, treats the Gaussian representation as an evolving physical system whose state evolves continuously under a learned motion law. This unlocks capabilities absent in deformation-based approaches:(1) sample-efficient learning from sparse temporal supervision by modeling the underlying motion law; (2) temporal extrapolation enabling forward and backward prediction beyond observed time ranges; and (3) compositional dynamics that allow localized dynamics injection for controllable scene synthesis. Experiments on dynamic scene benchmarks show that EvoGS achieves better motion coherence and temporal consistency compared to deformation-field baselines while maintaining real-time rendering

==> sec/3_old_method.tex <==
% \section{$M$-Planes (Motion Planes)}
% \label{sec:method}

% We aim to learn a time-varying $4D$ radiance field defined over $\textbf{q} = (x, y, z, t)$, but with a factorized representation and a warping mechanism that allows both coordinate-space and feature-space transitions. Our method comprises of (1) a $4D$ extension of tri-planes that factorizes $x, y, z, t$ into $ \binom{4}{2} = 6 $ planes, (2) a warp field that can be applied in either (a) coordinate space (\S\,\ref{subsec:coord_warp}) or (b) feature space (\S\,\ref{subsec:feat_warp}), and a (3) decoder (\S\,\ref{subsec:decoder}) to produce density $\sigma(\textbf{q})$ and color $c(\textbf{q}, \textbf{d})$. We detail each component and the loss functions that couple them below.

% \subsection{Overview of $m$-planes}
% \label{subsec:overview_mplanes}
% \vspace{-5pt}
% \paragraph{Motivation.} Typically, extending static radiance fields (e.g.\ NeRF~\cite{Mildenhall20}) to dynamic 4D data (with dimension $x, y, z, t$) often requires large neural networks~\cite{Gao21_DyNeRF} or storing separate parameters for each timestep. The result is high memory and runtime costs~\cite{Chen22_NeRFPlayer, Gao21_DyNeRF}. Factorized representations like TensoRF\cite{Chen22_Tensorf} or hexplanes\cite{Cao2023HEXPLANE} have shown that decomposing volumetric data into multiple lower-dimensional planes can be memory- and compute-efficient along with being interpretable. Building on these ideas, we propose $m$-planes as an extension of tri-planes that factors sapce and time into six planes--and pairs them with a small warp module to capture scene dynamics. This lets us \textbf{``roll forward"} (\cref{fig:roll_forward}(c))  the scene without retraining fresh parameters at each new timestep, thereby facilitating extrapolation to unseen frames with minimal overhead along with interpolating potential unseen frames. 

% \par \noindent {\bf High-Level Factorization.}  
% \label{subsec:factored}
% Following prior works on factorized representations~\cite{kplanes_2023, Cao2023HEXPLANE}, 
% we decompose the 4D coordinate \(\bm{q} = (x, y, z, t)\) into a minimal set of planes that capture pairwise interactions between dimensions. 
% Analogous to tri-plane factorization in 3D~\cite{Muller22_instantNGP, Chen22_Tensorf}, we construct a \emph{six-plane} factorization for 4D, consisting of three \emph{spatial} planes (\(\mathbf{P}_{xy}, \mathbf{P}_{xz}, \mathbf{P}_{yz}\)) and three \emph{spatiotemporal} planes (\(\mathbf{P}_{xt}, \mathbf{P}_{yt}, \mathbf{P}_{zt}\)).  
% Each plane is a learned 2D feature grid of shape \(N \times N \times M\), where \(N\) is the resolution per axis, and \(M\) is the feature dimension.

% \par \noindent {\bf Feature Extraction.} 
% \label{subsec:feat_extract}
% To obtain features for a query point \(\bm{q} = (x, y, z, t) \in \mathbb{R}^4\), we first normalize \(\bm{q}\) into the range \([0, N)\), then project ($\pi$) it onto each plane ($c$).  
% For a given plane \(\mathbf{P}_{c}\), we compute:
% $
% f_{c}(\bm{q}) = \psi\bigl(\mathbf{P}_{c}, \pi_{c}(\bm{q})\bigr),$
% where \(\pi_{c}(\bm{q})\) denotes the projection of \(\bm{q}\) onto plane \(\mathbf{P}_{c}\), and \(\psi\) is bilinear interpolation.  
% This process is repeated across all six planes, yielding six feature vectors, which we then combine via an elementwise Hadamard product:  
% \begin{equation}
% \label{eq:hadamard_planes}
% f(\bm{q}) = \bigcup\limits_{s \in S} \prod\limits_{c \in C} \psi(\mathbf{P}_c^s, \pi_c(\bm{q})).
% \vspace{-3mm}
% \end{equation}
% Here, \(\bigcup\) represents concatenation across multiple scales, allowing the model to capture features at different resolutions, while the Hadamard product ensures localized spatial-temporal expressivity, $C = \{xy,xz,yz,xt,yt,zt\}$, and $S$ is the set of scales used in multi-scale feature concatenation.

% \noindent As in prior works~\cite{Cao2023HEXPLANE, kplanes_2023}, this multiplicative fusion improves local expressivity, allowing each plane to act as a selector in localized spatiotemporal regions. The resulting feature vector \( f(\bm{q}) \in \mathbb{R}^M \) is then decoded into density \(\sigma(\bm{q})\) and view-dependent color \( \mathbf{c}(\bm{q}, \mathbf{d}) \).


% \par \noindent {\bf Local Feature Assembly.}
% When we sample a batch of \(C\) rays (chunk size),
% each with \(N\) points along it, we obtain
% \(\{ \bm{q}^i \}_{i=1}^{C\times N}\).
% Applying the above interpolations, we gather the plane features into a
% tensor of shape \(\bigl(C,\,N,\,6,\,M\bigr)\) (or equivalent), where
% “6” indexes the plane \(\mathbf{P}_{xy}, \mathbf{P}_{xz}, \dots, \mathbf{P}_{zt}\).
% We then combine these 6 plane features by an elementwise multiplication (Hadamard product) as shown in \cref{eq:hadamard_planes} yielding a final feature \(f(\bm{q}) \in \mathbb{R}^M\) of shape \(\bigl(C,\,N,\,M\bigr)\).

% \par \noindent {\bf Scene-Level Aggregation.}
% \label{subsec:scene_level_aggr}
% When performing feature-space warping or building a global scene descriptor, we merge the per-point features 
% \(\{f(\bm{q}^i)\}_{i=1}^{C \times N}\) into a single vector \(\bm{z}\). Specifically, we define an aggregator:
% \[
% \bm{z} = \mathcal{A}\Bigl(\{\, f(\bm{q}^i) \bigr\}_{i=1}^{C \times N}\Bigr) \;\in\;\mathbb{R}^{D},
% \]
% where \(D\) can be equal to \(M\) (in a simple pooling scenario) or differ if the aggregator changes dimensionality. We explore: \textbf{(1)} Average pooling: \(\bm{z} = \tfrac{1}{C \times N} \sum_{i} f(\bm{q}^i),\) typically preserving \(D = M\). \textbf{(2)} Max pooling: \(\bm{z}_j = \max_{i}\bigl[f(\bm{q}^i)\bigr]_j,\) also typically resulting in \(D = M\). \textbf{(3)} MLP aggregation: each \(f(\bm{q}^i)\in\mathbb{R}^M\) passes through a small MLP that may reduce or expand the feature dimension, then we pool or concatenate outputs to form \(\bm{z}\in\mathbb{R}^D\). We provide ablations for these methods in ~\cref{tab:mplanes_ablation} and ~\cref{fig:feat_aggr}.
% In practice, simple average pooling often suffices for scenes with relatively uniform features, while more complex aggregators can improve expressiveness for larger or highly diverse scenes. We view \(\bm{z}\) as a \textit{scene code} summarizing the geometry and appearance in the chunk. In \S\ref{subsec:warp_field}, we describe how we can either warp coordinates in \(\mathbb{R}^3\) or warp these global features \(\bm{z}\in\mathbb{R}^D\) to predict future frames or unobserved timesteps.

% \par \noindent {\bf Decoder.} 
% \label{subsec:decoder}
% We follow the decoding strategies of Hexplane~\cite{Cao2023HEXPLANE} and other factorized methods 
% (e.g.~TensoRF~\cite{Chen22_Tensorf}) to map our $M$-dimensional feature  $f(\bm{q})$ to density $\sigma(\bm{q})$ and view-dependent color $\mathbf{c}(\bm{q}, \mathbf{d})$.
% Two variants are supported: (1) we interpret $f(\bm{q})$ as coefficients for a learned basis (similar to NeX~\cite{wizadwongsa2021nex}), resulting in explicit dot products for color and density and (2) A small MLP ingests $f(\bm{q})$ and optionally the embedded direction $\gamma(\mathbf{d})$ to predict $(\sigma, \mathbf{c})$, akin to Instant-NGP~\cite{Muller22_instantNGP} or DVGO~\cite{Sun22_DVGO}. In both cases, we ensure $\sigma(\bm{q})\!>\!0$ and $\mathbf{c}\!\in\![0,1]$ 
% via standard activations (e.g.\ exponential, sigmoid). 
% We refer readers to \cite{Chen22_Tensorf, kplanes_2023} 
% for the implementation details on these decoders.

% \vspace{-3pt}
% \subsection{Warp Field}
% \label{subsec:warp_field}

% We propose two strategies for capturing how the scene evolves from one timestep to the next: 
% \emph{(a) coordinate-space warp} and \emph{(b) feature-space warp}. Both rely on lightweight MLP \(w_\theta\) that takes either coordinates \((\bm{q}, t)\) or scene features 
% \((\bm{z}_t, t)\), along with a positional (Fourier) encoding~\cite{Mildenhall20}, to output a displacement 
% (or directly predict the next state). We jointly optimize this MLP with our $m$-planes representation to ensure 
% temporal coherence in the learned dynamic scene.

% \par \noindent {\bf (a) Coordinate-Space Warp.}
% \label{subsec:coord_warp}
% In the coordinate-space warp, we predict a point displacement \(\Delta \bm{q}\) at time \(t\):
% \[
% \Delta\bm{q} \;=\; w_\theta\bigl(\gamma(\bm{q}),\,\gamma(t)\bigr) \quad
% \Longrightarrow \quad 
% \bm{q}_{t+1}^\mathrm{pred} \;=\; \bm{q}_t + \Delta\bm{q},
% \]
% where \(\bm{q}_t\in\mathbb{R}^3\) is a sampled 3D point at time \(t\), and 
% \(\gamma\) denotes a positional encoding that expands each coordinate or time scalar into a higher-dimensional frequency space.  
% For each sampled point, we also have (or approximate) the ground-truth position \(\bm{q}_{t+1}\) at time \(t+1\).  
% To align the warped point with actual geometry at \(t+1\), we enforce that $m$-planes features at \(\mathbf{q}_{t+1}^\mathrm{pred}\) match those 
% at the true \(\bm{q}_{t+1}\):
% \[
% \mathcal{L}_{\text{warp-coord}} 
% \;=\;\sum_{\mathbf{q}_t \,\in\, \mathcal{B}}
% \Bigl\|\,
% f(\mathbf{q}_{t+1})
% \;-\;
% f(\mathbf{q}_{t+1}^{\mathrm{pred}})
% \Bigr\|^{2}.
% \]
% where \(f(\cdot)\) denotes our representation (~\cref{fig:roll_forward}). This penalty encourages \(w_\theta\) 
% to produce displacements that correctly map \(\bm{q}_t\) onto its location at time \(t+1\).

% \begin{figure*} % [t] means "top of the page"
%     \centering
%     % Insert your graphic. Use the correct path/filename extension.
    
%     \caption{\textbf{We evaluate our approach under three different settings} \textbf{(a)} Full-Supervision Training: The model is trained with all available frames as in prior dynamic view synthesis works like \cite{Gao21_DyNeRF, Cao2023HEXPLANE, kplanes_2023, li2022neural, mildenhall2019local, lombardi2019neural} \textbf{(b)} Sparse Frame Reconstruction: A subset of frames is removed, so the model can infer missing timesteps. \textbf{(c)} Future Scene Extrapolation: The model is trianed on only the first half of the sequence and tested on predicting the unseen future frames.}
%     \includegraphics[width=\linewidth]{figures/phase_a.pdf}
%     \vspace{-20pt}
%     \label{fig:roll_forward}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \caption{\textbf{Effect of missing timesteps on reconstruction quality} Our approach, evaluated with different warp strategies. Without Fourier features, the model struggles to generalize motion. Feature-space and coordinate-space warping improves continuity and achieve good reconstruction fidelity, particularly for fine details such as the salmon and hand motion.  }
%     \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/figures/result_2.pdf}
%     \includegraphics[width=\linewidth]{figures/result.pdf}
%     \label{fig:syn_results}
%     \vspace{-30pt}
% \end{figure*}


% \par \noindent {\bf (b) Feature-Space Warp.}
% \label{subsec:feat_warp}
% Alternatively, we can \emph{first} extract or aggregate per-point features 
% \(f(\bm{q}_t, t)\) into a scene-level feature \(\bm{z}_t\) (\S\ref{subsec:scene_level_aggr}).  
% We then apply our warp function:
% \[
% \Delta \bm{z} 
% \;=\;
% w_\theta\bigl(\gamma(\bm{z}_t),\,\gamma(t)\bigr),
% \quad \Longrightarrow \quad 
% \hat{\bm{z}}_{t+1} 
% \;=\;
% \bm{z}_t + \Delta \bm{z},
% \]
% which evolves the global feature descriptor forward in time.  
% (One may also define \(\hat{\bm{z}}_{t+1} = w_\theta\bigl(\gamma(\bm{z}_t),\,\gamma(t)\bigr)\) \emph{without} addition;  
% we found an additive update can stabilize training by predicting changes relative to \(\bm{z}_t\).)

% \noindent In practice, feature-space warping can be more robust for large or occluded motions, 
% since the warp now acts on a lower-dimensional code rather than on every 3D point.  
% We ensure \(\hat{\bm{z}}_{t+1}\) matches the aggregated code \(\bm{z}_{t+1}\) at time \(t+1\), e.g.:
% \[
% \mathcal{L}_{\text{warp-feat}} 
% \;=\;
% \sum_{t}\;
% \bigl\|\,
% \bm{z}_{t+1} 
% \;-\;
% \hat{\bm{z}}_{t+1}
% \bigr\|^2.
% \]
% Here, \(\bm{z}_{t+1}\) is aggregated from \(\ \mathcal{A}\Bigl(\{f(\bm{q}_{t+1}^i)\}_{i=1}^{C\times N}\Bigr)\). 
% We embed either \((\bm{q}, t)\) or \((\bm{z}_t, t)\) 
% with the same frequency-based encoding \(\gamma(a)= \{\sin(2^k a), \cos(2^k a)\}\)~\cite{Mildenhall20, tancik2020fourfeat} so that \(w_\theta\) can capture high-frequency variations. Ultimately $\mathcal{L}_f$ or $\mathcal{L}_\text{warp}$ is either the $\mathcal{L}_\text{warp-coord}$ or $\mathcal{L}_\text{warp-feat}$


% \subsection{Optimization}

% \noindent
% \textbf{Overall Objective.}
% We represent a dynamic 3D scene with our factorized $m$-planes (Sec.~\ref{subsec:factored}), using photometric supervision plus a warp loss (Sec.~\ref{subsec:warp_field}) to enforce consistency across time. Concretely, we render each training ray \(\mathbf{r}\in \mathcal{R}\) by querying per-point density \(\sigma\) and color \(\mathbf{c}\), then apply standard volumetric compositing to obtain a predicted color \(C(\mathbf{r})\). We penalize the L2 distance to the ground-truth color \(\hat{C}(\mathbf{r})\). Additionally, we incorporate warp constraints from either coordinate-space, or feature-space.
% \[
% \mathcal{L}
% \;=\;\!\frac{1}{|\mathcal{R}|}\,\sum_{\mathbf{r}\in \mathcal{R}}
% \bigl\|\,C(\mathbf{r})\,-\,\hat{C}(\mathbf{r})\bigr\|^2
% \;+\;\lambda_{\mathrm{warp}}\,\mathcal{L}_{\mathrm{warp}}
% \;+\;\lambda_{\mathrm{reg}}\,\mathcal{L}_{\mathrm{reg}},
% \]
% where \(\lambda_{\mathrm{warp}}, \lambda_{\mathrm{reg}}\) balance warp constraints and additional regularizers.

% \noindent
% \textbf{Color Regression.}
% To produce per-ray colors quickly, we follow the implementation of \cite{Cao2023HEXPLANE}. First, we query a density value \(\sigma\) from density planes for each sampled point, skip those with low opacity multiply with a small density basis matrix\cite{Cao2023HEXPLANE}. For color, we fetch an appearance feature \(\mathbf{f}\) from a appearance planes. We feed \(\mathbf{f}\) and the viewing direction \(\mathbf{d}\) into a small MLP to output RGB color \(\mathbf{c}\), for the predicted points, we use the view direction of the current view point. Alternatively, one may use an explicit basis approach (e.g.\ Spherical Harmonics~\cite{yu2021plenoctrees, wizadwongsa2021nex}) for color decoding, removing the MLP altogether at some fidelity cost. Either variant ensures \(\sigma(\mathbf{q})>0\) and \(\mathbf{c}(\mathbf{q}, \mathbf{d})\in[0,1]\) via standard activations (e.g.\ exponential, sigmoid).

% \noindent {\bf Viewpoint Assumption for Warped Points.}
% In our coordinate-space warp, we do not explicitly need a camera viewpoint when predicting a displacement 
% $\Delta \mathbf{q}$. However, if we want to decode color (or compare features) at the warped position 
% $\mathbf{q}_{t+1}^{\mathrm{pred}}$, we assume the same camera/viewpoint as the ground-truth frame $\mathbf{q}_{t+1}$.
% This is necessary to ensure the predicted point aligns with a known target color or feature, rather than introducing ambiguity by switching to a different camera. During training, we typically sample one viewpoint for frames $t$ and $t+1$, warp each 3D point from $t$ to $t+1$, and supervise against the corresponding color/feature at $t+1$. Although it might be possible to project the warped point into a novel camera or handle multi-camera scenarios, 
% staying within the same viewpoint provides a consistent supervision signal for learning the warp.

% \noindent \textbf{Regularization.}
% As noted in prior works~\cite{Cao2023HEXPLANE, kplanes_2023}, reconstructing dynamic scenes from sparse viewpoints is ill-posed, so additional constraints are crucial. We apply the same total variation (TV)~\cite{Chen22_Tensorf, Cao2023HEXPLANE} on the $m$-plane grids to enforce spatiotemporal smoothness, we also adopt depth consistency~\cite{niemeyer2022regnerf} to reduce artifacts in fast-moving or partially observed regions.

% \noindent \textbf{Coarse-to-Fine Training.}
% We employ a progressive upsampling strategy~\cite{Chen22_Tensorf, yu2021plenoctrees}, where the grid resolution for each plane is gradually increased during training. This accelerates early optimization (fewer parameters at first) and provides an implicit regularization by focusing on coarse geometry before refining high-frequency details.




% % $f(\bm{q}_{t}) = \bigcup\limits_{s \in S} \prod\limits_{c \in C} \psi(\mathbf{P}_c^s, \pi_c(\bm{q}_{t})) $ \\

% % $\bm{q}_{t+1}^{\text{pred}} = \bm{q}_t + w_\theta(\bm{q}_t, t) $ \\

% % $f(\bm{q}_t) = \bigcup\limits_{s \in S} \prod\limits_{c \in C} \psi(\mathbf{P}_c^s, \pi_c(\bm{q}_t))$

% % $\Delta\bm{q}_t$

% % \bigl(\underbrace{f_{xy}(\bm{q}) \odot f_{xz}(\bm{q}) \odot f_{yz}(\bm{q})}_{\text{space planes}}\bigr)
% % \odot
% % \bigl(\underbrace{f_{xt}(\bm{q}) \odot f_{yt}(\bm{q}) \odot f_{zt}(\bm{q})}_{\text{space--time planes}}\bigr)

==> tables/full_width_future.tex <==
% \begin{table*}[t!]
%     \centering
%     \caption{
%     \textbf{Future frame prediction on the DyNeRF ``cut roasted beef'' scene.}
%     Additional results for other scenes and datasets are reported in the supplementary material.
%     }
%         % We highlight \bestcell{best} and \secondcell{second} cells.}
%     \vspace{-1mm}
%     \resizebox{0.96\textwidth}{!}{
%     \begin{tabular}{p{3cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}}
%     \toprule[2pt]
%      & \multicolumn{3}{|c|} {$k\ge0.75$} & \multicolumn{3}{c|}{$k\ge0.5$} & \multicolumn{3}{c}{$k\ge0.25$} \\
%     Model & PSNR$\uparrow$  & D-SSIM$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$  & D-SSIM$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$  & D-SSIM$\downarrow$ & LPIPS$\downarrow$ \\
%     \midrule
%     HexPlane~\cite{Cao2023HEXPLANE} & - & - & - & - & - & - & - & - & - \\  
%     KPlane~\cite{kplanes_2023}  & - & - & - & - & - & - & - & - & - \\     
%     % Static TensoRF \\
%     % \midrule
%     4DGS~\cite{Wu2024_4DGaussianSplatting} & - & - & - & - & - & - & - & - & - \\  
%     % HexPlane\dag & 350k &29.182 & 0.021& \secondcell{0.089} & \secondcell{8.08}& \bestcell{6h} &\bestcell{224 $\times$}\\
%     \midrule
%     Ours & - & - & - & - & - & - & - & - & - \\  
%     % HexPlane\dag-all & 350k &31.615 &0.015 & 0.079 &8.41&6h &224$\times$\\
%     \bottomrule [2 pt]
%     \end{tabular}}
%     \label{tab:results_table}
% \end{table*}

==> tables/missing_timestep.tex <==
\begin{table}[t!]
    \centering
    \caption{
        \textbf{Ablation on integration methods under missing-frame interpolation.}
        RK4 outperforms Euler on the ``cut roasted beef". with smoother interpolation and higher reconstruction fidelity.
        }
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{p{3.5cm} P{1.3cm} P{1.3cm} P{1.3cm} P{1.3cm} }
    \toprule[2pt]
    Model &PSNR$\uparrow$  &SSIM $\uparrow$ & LPIPS_a $\downarrow$ & LPIPS_v$\downarrow$\\
    \midrule
    4DGS~\cite{Wu2024_4DGaussianSplatting} & - & - &- & - \\
    \textbf{Ours} (Euler) & - & - & - & - \\  
    \textbf{Ours} (RK4) & - & - & - & -  \\  
    \bottomrule [2 pt]
    \end{tabular}}
    \label{tab:missing_timestep}
\end{table}




==> tables/mplane_ablation.tex <==
\begin{table}[t!]
    \centering
    \caption{
        \textbf{Ablations on  $m$-plane feature aggregation.}
        We compare three strategies for aggregating local features into a global representation 
        (\textit{Max-pool}, \textit{Average-pool}, and \textit{MLP aggregation}) on the Plenoptic Video dataset~\cite{li2022neural}. 
        Metrics include PSNR, SSIM, and LPIPS, where \textit{LPIPS\(_a\)} is computed using an AlexNet backbone, 
        and \textit{LPIPS\(_v\)} is computed using a VGG backbone.
        Results show that an MLP-based aggregator yields the best reconstruction quality, 
        while simpler pooling methods result in lower fidelity and higher perceptual error.
        }
        

    \vspace{-2mm}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{p{3.2cm} P{1.3cm} P{1.3cm} P{1.3cm} P{1.3cm} }
    \toprule[2pt]
    Model Variant &PSNR$\uparrow$  & SSIM$\uparrow$ & LPIPS_a$\downarrow$ &LPIPS_v$\downarrow$\\
    \midrule
    Max-pool  &24.39 &0.816 & 0.239 & 0.334 \\ 
    Average-pool & \secondcell{29.71} & \secondcell{0.883} & \secondcell{0.209} & \secondcell{0.326}\\
    MLP aggregation & \bestcell{31.30} & \bestcell{0.931} & \bestcell{0.093} & \bestcell{0.202}\\  
    \bottomrule [2 pt]
    \end{tabular}}
    \label{tab:mplanes_ablation}
\end{table}


==> tables/plenoptic_full_train.tex <==
\begin{table}[t!]
    \centering
    \caption{
        \textbf{Comparison with dynamic scene representations on the Neural 3D Video dataset.}
        \texttt{EvoGS} achieves the highest reconstruction fidelity and temporal stability while converging an order of magnitude faster 
        than deformation- or frame-based baselines. All methods are trained under identical view and frame sampling conditions.
        }
    \vspace{-2mm}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{p{3.5cm} P{1.3cm} P{1.3cm} P{1.3cm} P{1.3cm}}
    \toprule[2pt]
    Model &PSNR$\uparrow$  &SSIM$\uparrow$ & LPIPS$\downarrow$ & Time$\downarrow$ \\
    \midrule
    3D-GS~\cite{li2022neural} & - &  & - & - \\
    K-Planes~\cite{kplanes_2023} & - & - & - & - \\
    HexPlane~\cite{Cao2023HEXPLANE} & - & - & - & - \\
    4DGS~\cite{Wu2024_4DGaussianSplatting} & - & - & - & - \\
    \midrule
    \textbf{EvoGS (Ours)} & \bestcell{-} & \bestcell{-} & \bestcell{-} & \secondcell{-} \\  
    \bottomrule[2pt]
    \end{tabular}}
    \label{tab:plenoptic}
\end{table}


==> tables/real_time.tex <==
\begin{table*}[t]
\centering
\caption{
\textbf{Rendering speed comparison on an NVIDIA L40 GPU.}
All scenes use matched Gaussian counts. 4DGS is faster due to direct deformation,
while \texttt{EvoGS} performs ODE integration but still reaches real-time.
}
\label{tab:fps_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Scene} & \textbf{Method} & \textbf{Gaussians} &
\textbf{Avg FPS}$\uparrow$ & \textbf{Render Time (ms)}$\downarrow$ & \textbf{Real-time} \\
\midrule

% ---------------- LEGO
Lego           & 4DGS & 85,468 & \textbf{232.06} & 4.31 & \textcolor{green}{\checkmark} \\
               & Ours & 85,468 & 67.13           & 14.90 & \textcolor{green}{\checkmark} \\
\midrule

% ---------------- MUTANT
Mutant         & 4DGS & 56,079 & \textbf{308.64} & 3.24 & \textcolor{green}{\checkmark} \\
               & Ours & 56,079 & 80.74           & 12.39 & \textcolor{green}{\checkmark} \\
\midrule

% ---------------- JUMPING JACKS
Jumping Jacks  & 4DGS & 33,226 & \textbf{356.46} & 2.81 & \textcolor{green}{\checkmark} \\
               & Ours & 42,018 & 88.16           & 11.34 & \textcolor{green}{\checkmark} \\
\bottomrule
\end{tabular}
}

\vspace{1mm}
\begin{flushleft}
\footnotesize  
\textbf{Setup:} NVIDIA L40 (48GB), 100-frame sweep, fixed camera.  
All methods satisfy real-time ($\geq$30 FPS).
\end{flushleft}
\end{table*}

==> tables/results.tex <==
% \begin{table*}[t!]
%     \centering
%     \caption{
%     \textbf{Quantitative Comparisons on Plenoptic Video dataset~~\cite{li2022neural}.}
%     We report synthesis quality, training times (measured in GPU hours) with speedups relative to DyNeRF~\cite{li2022neural}.
%     With $672\times$ speedups, HexPlane\dag  with fewer training iterations  has comparable quantitative results to DyNeRF.
%     And HexPlane trained with the same iterations noticeably outperforms DyNeRF.
%     Baseline methods are evaluated on a particular scene, and we also report average results on all public scenes~(\emph{-all}). 
%     \colorbox{lightyellow}{Best} and \colorbox{lightgray}{Second} results are in highlight.}
%         % We highlight \bestcell{best} and \secondcell{second} cells.}
%     \vspace{-1mm}
%     \resizebox{0.96\textwidth}{!}{
%     \begin{tabular}{p{3cm} P{1.5cm}  P{1.5cm}  P{1.5cm} P{1.5cm} P{1.5cm} P{2.5cm} P{2.0cm}}
%     \toprule[2pt]
%     Model &Steps & PSNR$\uparrow$  & D-SSIM$\downarrow$ & LPIPS$\downarrow$ & JOD $\uparrow$ &Training Time$\downarrow$ &Speeds-up $\uparrow$\\
%     \midrule
%     Neural Volumes~\cite{lombardi2019neural} &- & 22.800 & 0.062 &0.295 &6.50 &- &-\\
%     LLFF~\cite{mildenhall2019local} & -&23.239  &0.076 &0.235 &6.48 &- &- \\
%     NeRF-T~\cite{li2022neural} & - &28.449 &0.023 &0.100 &7.73 & - & - \\
%     DyNeRF~\cite{li2022neural}  &650k  & \bestcell{29.581} & \secondcell{0.020} & 0.099 & 8.07 &1344h &1$\times$ \\    
%     % Static TensoRF \\
%     % \midrule
%     HexPlane & 650k &\secondcell{29.470} & \bestcell{0.018} &\bestcell{0.078} & \bestcell{8.16} &\secondcell{12h} & \secondcell{$112 \times$}\\
%     % HexPlane\dag & 350k &29.182 & 0.021& \secondcell{0.089} & \secondcell{8.08}& \bestcell{6h} &\bestcell{224 $\times$}\\
%     HexPlane\dag & 100k & 29.263 & \secondcell{0.020} & \secondcell{0.097} &\secondcell{8.14} & \bestcell{2h} & \bestcell{672} $\times$ \\
%     \midrule
%     HexPlane-all & 650k &31.705 &0.014 & 0.075 & 8.47 & 12h & 112 $\times$\\  
%     HexPlane\dag-all & 100k & 31.569 & 0.016 &0.089 & 8.36 & 2h & 672 $\times$ \\
%     % HexPlane\dag-all & 350k &31.615 &0.015 & 0.079 &8.41&6h &224$\times$\\
%     \bottomrule [2 pt]
%     \end{tabular}}
%     \label{tab:results_table}
%     \vspace{-4mm}
% \end{table*}
